ControlNET: A Firewall for RAG-based LLM System

Retrieval-Augmented Generation (RAG) has significantly enhanced the factual accuracy and domain adaptability of Large Language Models (LLMs). This advancement has enabled their widespread deployment across sensitive domains such as healthcare, finance, and enterprise applications. RAG mitigates hallucinations by integrating external knowledge, yet introduces privacy risk and security risk, notably data breaching risk and data poisoning risk. While recent studies have explored prompt injection and poisoning attacks, there remains a significant gap in comprehensive research on controlling inbound and outbound query flows to mitigate these threats. In this paper, we propose an AI firewall, ControlNET, designed to safeguard RAG-based LLM systems from these vulnerabilities. ControlNET controls query flows by leveraging activation shift phenomena to detect adversarial queries and mitigate their impact through semantic divergence. We conduct comprehensive experiments on four different benchmark datasets including Msmarco, HotpotQA, FinQA, and MedicalSys using state-of-the-art open source LLMs (Llama3, Vicuna, and Mistral). Our results demonstrate that ControlNET achieves over 0.909 AUROC in detecting and mitigating security threats while preserving system harmlessness. Overall, ControlNET offers an effective, robust, harmless defense mechanism, marking a significant advancement toward the secure deployment of RAG-based LLM systems.

==> review.tex <==
Review of "\projectname: A Firewall for RAG-based LLM System"
This paper presents an innovative and much-needed approach to enhancing the security and privacy of Retrieval-Augmented Generation (RAG)-based Large Language Models (LLMs). The authors systematically address significant vulnerabilities in RAG systems, particularly those associated with data breaches and data poisoning. Through a detailed analysis of five distinct attack vectors—reconnaissance, data exfiltration, unauthorized access, knowledge poisoning, and conversation hijacking—the paper provides a comprehensive framework that effectively identifies and mitigates these risks. The proposed solution, \projectname, introduces a novel AI firewall that utilizes activation shift phenomena to detect and control malicious query flows. The paper’s approach stands out by proposing a mechanism that not only enhances security but also preserves the integrity and privacy of interactions within RAG-based LLM systems.

The strengths of the paper are evident in its contributions. First, the comprehensive risk analysis provides a well-structured taxonomy for categorizing privacy and security vulnerabilities, a valuable framework for future research. The introduction of \projectname represents a significant advancement in query flow control, demonstrating the ability to detect malicious queries based on distinct activation vector patterns. Additionally, the paper's rigorous experimental validation on state-of-the-art LLMs and diverse benchmark datasets, such as MS MARCO, HotpotQA, FinQA, and MedicalSys, substantiates the effectiveness of \projectname in mitigating privacy and security risks. The results, showcasing an AUROC exceeding 0.909 for risk detection, with minimal degradation in Precision and Recall, further underline the robustness of the proposed method. Furthermore, the inclusion of a multi-role medical database as an open-access benchmark will undoubtedly contribute to further research in this critical domain. These contributions not only make the paper an important advancement in the field of AI security but also position it as a key reference for the future design of secure RAG-based systems.

The paper's contributions are highly valuable, both in terms of theoretical advancements and practical applications. It addresses critical issues in RAG-based LLM systems and offers a solution that is both novel and practical. The robustness of the experimental results, coupled with the innovative proposal of \projectname, is impressive. Given the increasing reliance on LLMs for sensitive applications, the necessity of ensuring privacy and security is paramount. This paper provides a timely solution and is deserving of acceptance at ACM CCS. Its novel contributions and comprehensive analysis make it an essential read for researchers and practitioners in the field of AI security. Therefore, I strongly recommend the paper for acceptance without any reservations.

==> static/backup/back.tex <==
\begin{comment}
To the best of our knowledge, there is currently no comprehensive research that addresses both the privacy and security risks associated with RAG in LLMs. 
Given these inherent vulnerabilities, there is an urgent need for robust security measures to mitigate the risks of knowledge leakage, poisoning, and conversation hijacking. These measures must effectively address both privacy and security concerns, protecting against malicious clients and unscrupulous knowledge providers. Ensuring the integrity and confidentiality of RAG-based LLM systems is crucial for maintaining their reliability and trustworthiness in real-world applications, necessitating the development and implementation of advanced security protocols and continuous monitoring mechanisms.
\end{comment}

==> static/backup/backup.tex <==
\begin{comment}
We propose a novel LLM guardrail that detects and mitigates malicious queries inspired by the firewall mechanisms in network security. Traditional firewalls rely on regular expression matching to control network traffic by defining patterns that, when matched, permit or deny access. However, the complexity and variability of semantic queries in LLMs make it impractical to rely on predefined textual patterns alone. To solve above challenge, we seek for catching query's patterns through the activation direction of LLM instead of the raw text.
Recent studies in activation engineering have explored the potential for controlling LLMs by introducing opposite activation vectors, often referred to as steering vectors. For instance, in a pair of prompts such as \underline{"I love talking about weddings"} and \underline{"I hate talking about weddings,"} the terms \underline{"love"} and \underline{"hate"} serve as steering prompts, guiding the model's output in opposing directions.
Nevertheless, in the context of malicious query detection and mitigation, there is typically no direct opposite activation vector available for a given query. 
Fortunately, our observation reveals that conversations on distinct topics exhibit distinct directions in their activation vectors, which can be effectively distinguished by leveraging anchor points as unit direction vectors. 
To tracking the direction deviation, we define the concept of \textbf{activation distortion} and propose the sematic anchors to tracking these deviation.
We term this phenomenon the \textit{activation distortion phenomenon}.
Our intuition is to control LLM generation through tracking its activation distortion.




We define acceptance rules for each role $u_{i}$, containing a series of question-knowledge documents pairs (we define as \textbf{sematic anchors} $\{\mathcal{Q}_{anc}^{u_{i}}, \mathcal{D}_{anc}^{u_{i}}\}$). 





We propose a novel mechanism inspired by principles of activation engineering technique, which utilizes sematic anchor-based direction vectors to detect and mitigate malicious queries through the identification of activation distortion phenomena. 
Recent studies in activation engineering have explored the potential for controlling LLMs by introducing opposite activation vectors, often referred to as steering vectors. For instance, in a pair of prompts such as \underline{"I love talking about weddings"} and \underline{"I hate talking about weddings,"} the terms \underline{"love"} and \underline{"hate"} serve as steering prompts, guiding the model's output in opposing directions. However, in the context of malicious query detection and mitigation, there is typically no direct opposite activation vector available for a given query. 

Nevertheless, our observation reveals that conversations on distinct topics exhibit divergent directions in their activation vectors, which can be effectively distinguished by leveraging anchor points as unit direction vectors. 
Drawing upon the concept of firewall mechanisms, we define acceptance rules for each role $u_{i}$, containing a series of question-knowledge documents pairs (we define as \textbf{sematic anchors} $\{\mathcal{Q}_{anc}^{u_{i}}, \mathcal{D}_{anc}^{u_{i}}\}$). 
Queries that fall outside of this acceptance rules are classified as potentially malicious and are therefore denied access. 
In essence, malicious queries are characterized by significant deviations in their activation vector direction when compared to benign queries. We term this phenomenon the \textit{activation distortion phenomenon}.
Our intuition is to control LLM generation through tracking its activation distortion.
\end{comment}
